Efficient Planning under Partial Observability with Unnormalized Q Functions and Spectral Learning

Learning and planning in partially-observable domains is one of the most difficult problems in reinforcement learning. Traditional methods consider these two problems as independent, resulting in a classical two-stage paradigm: first learn the environment dynamics and then plan accordingly. This approach, however, disconnects the two problems and can consequently lead to algorithms that are sample inefficient and time consuming. In this paper, we propose a novel algorithm that combines learning and planning together. Our algorithm is closely related to the spectral learning algorithm for predicitive state representations and offers appealing theoretical guarantees and time complexity. We empirically show on two domains that our approach is more sample and time efficient compared to classical methods.

==> related_work.tex <==
should focus on the multi-task part
\begin{itemize}
    \item Introduce PSRs, TPSRs and its corresponding planning method: PBVI/fitted Q with extra tree etc. Highlight its drawback, i.e. doesn't connect with the reward function, thus the learned representation is disjoint from the planning part.
    \item Successor features, indicating its drawback, i.e. assume completely shared environment.
    \item other multi-task rl algorithms? (maybe not necessary, just focus on the linear case)
\end{itemize}
One of the challenges in model-based reinforcement learning consists in estimating the transition dynamics of a environment. In the case where states of the system are unknown and the agent has only access to observations generated under some fixed policy, the problem reduces to solving for the parameters of a partially observable Markov decision process (POMDP), i.e. the belief state transition function and the reward function.
It has been shown \citep{littman2002predictive} that in order to fully capture the environment model, it is sufficient to maintain a set of action-observation sequences known as \textit{predictive state representations} (PSRs). In their linear form, PSRs have been used in transfer learning \citep{sekharan2017transfer}, in which tests $t_1,...,t_n$ from a source task observed after some history $h$ are mapped onto a target task through a projection matrix linking transition models in both environments. In a non-linear setting, PSRs have been successfully applied to recurrent neural architectures and demonstrated desirable properties such as faster convergence rate \citep{venkatraman2017predictive,downey2017predictive}.\\

Traditionally, POMDPs have been analyzed and approximately solved using latent variable models, such as Hidden Markov models. A natural generalization of an HMM arises from the relaxation of the probability constraint on the belief transition function, and is known as a weighted finite-state automaton (WFA). Weighted automata are widely used to formalize the processing of sequential data in tasks such as string parsing and natural language understanding. Under the probabilistic setting, one can use the expectation-maximization algorithm to recover the corresponding WFA. However, this approach often suffers from local minimum problem. Spectral learning, on the other hand, does not rely on a probabilistic formulation and successfully avoids the local minimum problem through leveraging the spectral decomposition and method of moments.\\

Based on spectral learning methods for HMMs, \citep{boots2011closing} proposed the \textit{transformed} PSR framework, within which each sequence is decomposed into a product of an initial belief vector with transition matrices associated to each symbol in the trajectory. Features found in such a way are consistent up to a change of basis and converge to the true parameters with increasing training set sizes. Planning can be done directly from TPSRs using a variant of point-based value iteration \citep{pineau2003point}, without the need to recover the transition and emission kernels.

While, traditionally, spectral decomposition techniques have been used to solve single tasks, recent work from \cite{rabusseau2017multitask} provided insight on extensions into the multi-task setting. Notably, jointly learning multiple (usually related) tasks allows to find an intermediate representation shared across all domains, which can then be transferred onto similar, but unseen domains.

% A counterpart of PSRs in the fully observable MDP setting is the concept of successor features \citep{barreto2017successor}. Choosing a successor feature factorization of the reward function over a set of tasks with shared dynamics allows the model to learn a common embedding component of the transition dynamics, as well as a task-specific embedding of the goal. This concept is very similar to WFA, where the common embedding corresponds to the representation of the past trajectories and the goal embedding function are essentially the termination function. In particular, within the MTL framework, the automaton might have multiple termination functions.\\



In this work, we propose a novel approach for discovering state value functions in reinforcement learning domains based on the recent advance in multi-task automata learning \citep{rabusseau2017multitask}. Although multi-task learning in PSRs setting is not completely new \citep{sekharan2017transfer}, to the best of our knowledge no work has yet approached multi-task reinforcement learning from a spectral learning perspective.\\

\paragraph{Multi-task learning and knowledge transfer.} The problem of jointly learning a set of related tasks often arises in sequential decision making. For example, a robot trained to navigate a closed room should, with minimal training data, adapt to changes in topology. Leveraging the degree of similarity between multiple tasks poses an issue for simple model-based methods in reinforcement learning, as they need to re-estimate model parameters for new tasks. One simple solution consists in assuming a linear factorization of the reward (and thus the state value function) into shared and task-specific components \citep{dayan1993improving}. These \textit{successor representations} of state have recently been used in multi-task learning, in which the term without any temporal dependency was assumed to contain  features of the goal state \citep{barreto2017successor}. Under that restriction, transferring the successor value function across tasks is equivalent to jointly learning a shared feature space of transitions, followed by a task-specific projection step.
